GSL: A Cryptographic Library for the strong RSA Graph Signature Scheme

Current cloud and network infrastructures do not employ privacy-preserving methods to protect their assets. Anonymous credential schemes are a cryptographic building block that enables the certification of data structures and prove properties over their representations without disclosing the innards of their data structures in zero-knowledge. The GRaph Signature (GRS) scheme enables the certification and proof methods to sign infrastructure topologies represented as graph data structures and use zero-knowledge to prove properties over their certificates. As such, they represent a powerful privacy-preserving method that proves properties over a signed topology graph to another party without disclosing the blueprint of its topology. In this paper, we report our efforts in designing, implementing and benchmarking a Graph Signature Library (GSL). GSL is a cryptographic library realized in Java that implements the graph signature scheme.

==> tikz/fig-grs-groups-tree.tex <==
\begin{tikzpicture} %[scale=0.51] 
\sffamily
% \ttfamily 
%\tikzset{ 
%  table/.style={
%    matrix of nodes,
%    row sep=0cm,
%    column sep=0cm,
%    nodes={rectangle, text width=1.1cm, align=center},
%    nodes in empty cells
%  },
%  comp/.style={draw, thick, minimum width=4mm, minimum height=1cm, fill=white!10},
%  title/.style={draw, fill=black!10, font=\LARGE\scshape,node distance=10pt, text=black!40, inner sep=1mm},
%  multimultinode/.style={comp, double copy shadow, fill=white},
%}
\begin{scope} %[xshift=-10cm]

\tikz \graph [tree layout, missing nodes get space,  minimum number of children=1, nodes={draw, fill=gray!50, thick,  rectangle}] { Groups -> { QRGroupN, QRGroupPQ, CommitmentGroup  }  };
\end{scope}

%\begin{scope} [xshift=-2cm]
%\tikz \graph [tree layout, missing nodes get space,  minimum number of children=1, nodes={draw, fill=black!50, thick,  rectangle}] { GroupElements -> { QRGroupN, QRGroupPQ, CommitmentGroup  }  };
%\end{scope}

\end{tikzpicture}

